Fast Prospective Detection of Contrast Inflow in X-ray Angiograms with Convolutional Neural Network and Recurrent Neural Network

Automatic detection of contrast inflow in X-ray angiographic sequences can facilitate image guidance in computer-assisted cardiac interventions. In this paper, we propose two different approaches for prospective contrast inflow detection. The methods were developed and evaluated to detect contrast frames from X-ray sequences. The first approach trains a convolutional neural network (CNN) to distinguish whether a frame has contrast agent or not. The second method extracts contrast features from images with enhanced vessel structures; the contrast frames are then detected based on changes in the feature curve using long short-term memory (LSTM), a recurrent neural network architecture. Our experiments show that both approaches achieve good performance on detection of the beginning contrast frame from X-ray sequences and are more robust than a state-of-the-art method. As the proposed methods work in prospective settings and run fast, they have the potential of being used in clinical practice.

==> discussion.tex <==
\section{Conclusion}
\label{sec:conclusion}
  

% also talk about the application of using the method
\noindent We have developed two types of approaches for online detection of contrast inflow in XA sequences, enhancement-based and learning-based. The proposed methods achieve good performances on BCF detection tasks in XA sequences, and outperform a previous state-of-the-art method. The two types of methods both work in online settings, therefore have the potential to be used during real clinical interventions.







